YETI follow-up observations of the T Tauri star CVSO30 with transit-like dips

The T Tauri star CVSO30, also known as PTFO8-8695, was studied intensively with ground based telescopes as well as with satellites over the last decade. It showed a variable light curve with additional repeating planetary transit-like dips every ~0.8h. However, these dimming events changed in depth and duration since their discovery and from autumn 2018 on, they were not even present or near the predicted observing times. As reason for the detected dips and their changes within the complex light curve, e.g. a disintegrating planet, a circumstellar dust clump, stellar spots, possible multiplicity and orbiting clouds at a Keplerian co-rotating radius were discussed and are still under debate. In this paper, we present additional optical monitoring of CVSO30 with the meter class telescopes of the Young Exoplanet Transit Initiative in Asia and Europe over the last seven years and characterize CVSO30 with the new Early Data Release 3 of the ESA Gaia Mission. As a result, we describe the evolution of the dimming events in the optical wavelength range since 2014 and present explanatory approaches for the observed variabilities. We conclude that orbiting clouds of gas at a Keplerian co-rotating radius are the most promising scenario to explain most changes in CVSO30's light curve.

==> mnguide.tex <==
% MNGUIDE.TEX
%
% Authors' guide for the plain TeX MN macros
%
% v1.6 --- released 18th September 1995 (A. Woollatt)
% v1.5 --- released 25th August 1994 (M. Reed)
% v1.4 --- released 22nd February 1994
% v1.3 --- released 21st December 1992
%
% Copyright Cambridge University Press

% The following line automatically loads the mn macros if you are not
% using a format file.
\ifx\mnmacrosloaded\undefined \input mn\fi

% If your system has the AMS fonts version 2.0 installed, MN.tex can be
% made to use them by uncommenting the line: %\AMStwofontstrue
%
% By doing this, you will be able to obtain upright Greek characters.
% e.g. \umu, \upi etc.  See the section on "Upright Greek characters" in
% this guide for further information.

\newif\ifAMStwofonts
%\AMStwofontstrue


%%%%%%%%%%%%%%%%%%%%%%%%% Macros for this guide %%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newskip\ttglue \ttglue=0pt

\chardef\other=12
\def\ttverbatim{\begingroup \catcode`\\=\other \catcode`\{=\other
 \catcode`\}=\other \catcode`\$=\other \catcode`\&=\other
 \catcode`\#=\other \catcode`\%=\other \catcode`\~=\other
 \catcode`\_=\other \catcode`\^=\other
 \obeyspaces \obeylines \tt}%
{\obeyspaces\gdef {\ }}

\outer\def\begintt{$$\let\par=\endgraf \ttverbatim \parskip=0pt%
 \catcode`\|=0 \rightskip=-5pc \ttfinish}

{\catcode`\|=0 |catcode`|\=\other
 |obeylines
 |gdef|ttfinish#1^^M#2\endtt{#1|vbox{#2}|endgroup$$}}

\catcode`\|=\active
{\obeylines\gdef|{\ttverbatim\spaceskip=\ttglue\let^^M=\ \let|=\endgroup}}

\newdimen\macind   \macind=1em % the default indent

\def\beginlines{\par\begingroup\nobreak\Half
  \leftskip=\macind
  \parindent=0pt%
  \nobreak \obeylines \everypar{\strut}%
}
\def\endlines{\endgroup\Half\noindent}

\def\hang#1#2{%
 \par\hangindent=70pt%
 \advance\hangindent by 1em
 \noindent\hskip 1em \rlap{\tt #1}\hskip 70pt\relax
 #2\par%
}

\def\beginexhang#1{\par\bgroup\let\item=\ex@hang}

\def\ex@hang#1{%
  \everypar{}\par
  \Half
  \everypar{\noindent \ignorespaces}%
  \noindent %\hskip-\hangindent
    \boxw{\tt\char"5C #1}\quad\ignorespaces
}

\def\endexhang{\par\egroup\Half}

\def\beginquote{\bgroup\par\Half\leftskip=2em \rightskip=2em
  \eightpoint\noindent\ignorespaces}
\def\endquote{\par\Half\egroup\noindent}

\newdimen\fboxrule \fboxrule=.4pt
\newdimen\fboxsep  \fboxsep=3pt
\newdimen\tempdimA
\newbox\BoxA

\newif\ifnocr
\def\boxw#1{{\global\nocrtrue \fboxsep=2pt \boxit{#1}}}

\long\def\boxit#1{%
  \setbox\BoxA=\hbox{\kern\fboxsep #1\kern\fboxsep}%
  \tempdimA=\fboxrule
  \advance\tempdimA by \fboxsep
  \advance\tempdimA by \dp\BoxA
  \noindent \hbox{\lower\tempdimA
  \hbox{%
    \vbox{%
      \hrule height \fboxrule
      \hbox{%
        \vrule width \fboxrule \hskip-\fboxrule
        \vbox{\vskip\fboxsep \box\BoxA\vskip.5\fboxsep}%
        \hskip -\fboxrule \vrule width \fboxrule
      }%
    \hrule height \fboxrule
    }%
  }%
  }%
  \ifnocr \global\nocrfalse\else \par\medskip\noindent\ignorespaces\fi
}

\def\multi{\vbox\bgroup\advance\hsize by -2\fboxsep \def\\{\hfil\break}}
\def\endmulti{\egroup}

\def\Notes{%
  \if@nobreak \everypar{}\half \else \addpen{\gds@cbrk}\addvspace{\half}\fi
  \noindent\@nohdbrk {\em Notes}\par
  \nobreak \vskip\half \nobreak \@noafterindent
}


\def\LaTeX{La\TeX}
\makeatother
%%%%%%%%%%%%%%%%%%%%%% End of macros for guide %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifCUPmtplainloaded \else
  \NewTextAlphabet{textbfit} {cmbxti10} {}
  \NewTextAlphabet{textbfss} {cmssbx10} {}
  \NewMathAlphabet{mathbfit} {cmbxti10} {} % for math mode
  \NewMathAlphabet{mathbfss} {cmssbx10} {} %  "   "    "
  %
  \ifAMStwofonts
    %
    \NewSymbolFont{upmath} {eurm10}
    \NewSymbolFont{AMSa} {msam10}
    \NewMathSymbol{\upi}     {0}{upmath}{19}
    \NewMathSymbol{\umu}     {0}{upmath}{16}
    \NewMathSymbol{\upartial}{0}{upmath}{40}
    \NewMathSymbol{\leqslant}{3}{AMSa}{36}
    \NewMathSymbol{\geqslant}{3}{AMSa}{3E}
    \let\oldle=\le     \let\oldleq=\leq
    \let\oldge=\ge     \let\oldgeq=\geq
    \let\leq=\leqslant \let\le=\leqslant
    \let\geq=\geqslant \let\ge=\geqslant
  \else
    \def\umu{\mu}
    \def\upi{\pi}
    \def\upartial{\partial}
  \fi
\fi

% Marginal adjustments using \pageoffset maybe required when printing
% proofs on a Laserprinter (this is usually not needed).
% Syntax: \pageoffset{ +/- hor. offset}{ +/- vert. offset}
% e.g.    \pageoffset{-3pc}{-4pc}

\pageoffset{-2.5pc}{0pc}
\overfullrule=0pt

\loadboldmathnames

\begintopmatter  %  start the two spanning material

\title{Monthly Notices of the Royal Astronomical Society:\hfil\break
  plain \TeX\ style guide for authors}
\author{M. A. Reed}
\affiliation{Cambridge University Press, Shaftesbury Road,
  Cambridge CB2 2BS}

\shortauthor{M. A. Reed}
\shorttitle{Monthly Notices: plain \TeX\ guide for authors}

\acceptedline{Accepted 1993 December 11. Received 1993 March 17}

\abstract {This guide is for authors who are preparing papers for the
Monthly Notices of the Royal Astronomical Society using the
Monthly Notices plain \TeX\ macros.}

\keywords {Plain \TeX, {\tt mn.tex} -- sample text -- user guide.}
\pagerange{1--13}%%
\pubyear{1994}

\maketitle

% Start of main text

\section{Introduction}

In addition to the standard submission of hardcopy from authors,
Monthly Notices accepts machine-readable forms of papers in \TeX.
The layout design for Monthly Notices has been implemented as a
\TeX\ format. This guide is not a substitute for the \TeX\ manual
itself. Authors planning to submit their papers in \TeX\ are advised
to use |mn.tex| as early as possible in the creation of their files.


\subsection{The MN macros}

MN is a set of plain \TeX\ macros for the Monthly Notices design,
incorporating both the single- and double-column formats.
MN.STY is the corresponding \LaTeX\ style file.
The MN design package consists of the following files; do not edit these
files in any way.
\Half
\hang{MN.TEX}       {the macro definitions}
\hang{MNGUIDE.TEX}  {the input file for this guide}
\hang{MNSAMPLE.TEX} {the input file for a sample article}
\hang{MNLAND.TEX}   {a landscape figure for use with the sample article}
\hang{FONTTEST.TEX} {a file to test all of the fonts used in MN}
\Half
\noindent The input files for the guide, sample pages, landscape sample and
fonttest automatically call in the MN macros if you haven't preloaded them
by using a format file.
Therefore, this guide can be typeset by typing: |tex MNGUIDE|, or
|tex &mn MNGUIDE|.

When your article is printed in the Monthly Notices journal, it is typeset
in Monotype Times. As most authors do not have this font, it is likely that
the make-up will change with the change of font. For this reason, we ask
you to ignore details such as slightly long lines, page stretching, or
figures falling out of synchronization, because these details can be dealt with at a later stage.


\subsection{General style issues}

For general style issues, authors are referred to the `Instructions for
Authors' on the inside back cover of Monthly Notices. Authors who are
interested in the details of style are referred to Butcher (1992) and
The Chicago Manual (1982). The language of the journal is British
English and spelling should conform to this.


\subsection{Submission of \TeX\ articles to the journal}

Authors are urged to state that electronic submission is intended when
first submitting their paper. Papers should initially be submitted in the
usual way to the Executive Secretary, Royal Astronomical Society, Burlington
House, London W1V~0NL, as set out on the inside front cover of each issue
of Monthly Notices. Three hard copies should be supplied. One of these
copies should be single-sided and double-spaced throughout, while the other
two should be weight-reduced, by being either single-spaced or double-sided.
Note that articles, or revised versions thereof, may not be submitted by
electronic mail.  Appropriate gaps should be left for figures, original
versions and copies of which should also be supplied.  Authors should ensure
that their figures are suitable (in terms of lettering, size, etc.) for the
reduction they intend.

Authors who wish to include PostScript artwork dir\-ectly into their
articles can do so, by using either Tomas Rokicki's {\sf EPSF} macros
or Trevor Darrell's {\sf PSFIG} macros (both of which are supplied with
the DVIPS PostScript driver). Please remember to supply any additional
figure macros you use with your article.
Please also supply hard copies of your figures, for the use of production
editors and as a back-up.
Authors should not attempt to
use implementation specific |\special|'s directly.

The correct Monthly Notices House
Style should be used -- details are given in the Instructions for Authors,
in the Style Guide published in the 1~January 1993 issue (\hbox{MNRAS},
260,~1), and in Appendix C of this guide.
No disk should be submitted at this initial stage. When the paper has been
accepted, the double-spaced copy will be marked up by the subeditors at
Blackwell Science (BS) and returned to you for correction.
When the requested corrections have been made, you should send the following
material to BS:
\beginlist
\item (i) a 3.5-inch or 5.25-inch disk for PC (double or high density or
Apple Mac), containing the {\em corrected\/} version of the paper; the file
for the final version should be text-only, with no source-dependent control
codes (i.e. an ASCII file);

\item (ii) two hard copies of the corrected version, plus the original
marked up copy of the article; {\em any further author corrections should
be clearly indicated on the latter\/};

\item (iii) a signed statement that the revised hard copy and the disk do
indeed correspond.
\endlist
In addition, you should submit the following information concerning the disk
and its contents:
\beginlist
\item (i) the disk format (e.g. PC 360k);

\item (ii) how many files the disk contains, their names, a description of
the file contents and the number of pages each file will produce when
printed; details of any user-defined macros;

\item (iii) the computer system and implementation of \TeX\ used (e.g.
IBM~PC-386, PC\TeX~v3.14).
\endlist
Unless the layout of the paper has to be significantly changed by the
typesetter (for example, if the gaps left for figures are not suitable), it
will not be necessary to send you a typeset proof to check, as the paper
will be set directly from your submitted disk.  However, you should note
that, if serious problems are encountered with the coding of your paper
(missing author-defined macros, for example), it may prove necessary to
divert the paper to conventional typesetting.


\section{General instructions for installation}

The simplest way to use this macro package is to copy the above files into a
suitable directory or work area on your computer.  Write your
article using the macros described below (or use the sample article as a 
template) and ensure that the following is included at the very beginning of your input file:
\beginlines
|\ifx\mnmacrosloaded\undefined \input mn\fi|
\endlines

When you typeset your article using |tex <article file name>| the macro
definitions will be loaded automatically before your text is processed.
This will happen rather slowly on a small computer and you may find it much
faster to work with the \TeX\ format file for the MN macros.
This can be created by using the program INITEX:
\beginlines
|initex &plain mn|
\endlines
This usage of this command will vary from one installation of \TeX\ to
another. In {\sc Unix} implementations of \TeX\ the `|&|' character must
be `escaped' with a `|\|` because it is a magic character,
e.g. |initex \&plain mn|.
In PC\TeX\ you type the following (seek local advice if you
are not sure how to use INITEX on your system):
\beginlines
|tex &plain mn /i|
\endlines

When the process is complete type |\dump| at the \TeX\ prompt.
This creates the format file |MN.FMT|.  Type the following command to
typeset your article:
\beginlines
|tex &mn <article file name>|
\endlines
\TeX\ will process your article at high speed.


\subsection{The font test and sample pages}

Once you have installed the MN macros, run the following test.  The file
|FONTTEST.TEX| produces a sample of each font size used in the MN design.
To use this do |tex FONTTEST| or |tex &mn FONTTEST| (after creating the
|MN.FMT| format file).
Preview the resulting |DVI| file on-screen and generate hard copy output on
your facilities.  It will show you whether any of the fonts selected by the
Monthly Notices design are going to cause problems on your system.

As a final test of the installation, typeset the sample article, using
|tex MNSAMPLE| or |tex &mn MNSAMPLE|.
Use this article in conjunction with the instructions in this guide to
work out how to typeset an article for Monthly Notices.


\subsubsection{Page margins}

Some \TeX\ sites may find that pages from the MN design are positioned
incorrectly on the paper from local laserprinters. This can be corrected by the
use of the |\pageoffset| macro. It takes two parameters, the first being
the horizontal offset, the second the vertical offset, e.g.
\beginlines
|\pageoffset{-1pc}{2pc}|
\endlines
The above example will shift the output one pica to the left, and two picas
down the page. Usually there is no need to use this macro; only use it if
required.


\subsubsection{Author macro names}

For efficiency, some authors may wish to write their own macros. Those who
intend to do this will be aware of the problem of creating unique
identifiers (macro names). The most common way around this problem has been
to include |@| somewhere in the identifier, e.g. |\@utput| or |\sec@tion|.
Knuth, the creator of \TeX, has adopted this method in the plain \TeX\
definitions and it can also be found in other format packages such as
\LaTeX.

However, use of this method can cause problems if the internals of plain
\TeX\ or the MN macros get `over-ridden'. There is a simpler method which is
much safer. Simply prefix your macro names with your initials,
e.g.\ |\MARmacro|.


\section{The design macros}

Refer to the source code of the sample pages for examples of the following
design macros in use. It is very important that the article should end
with a |\bye| as this typesets `This paper$\ldots$' at the very end.


\subsection{Article opening}

There are certain macros that should appear near the top of your input file.
The following is the recommended way to begin your article.
%
\beginexhang{begintopmatter}
\item{onecolumn} Selects single-column output (default = two-column).
  The |\onecolumn| command {\em must\/} be used before |\begintopmatter|
  for the article opening to work correctly.

  You should not use |\onecolumn| unless your article has a high
  mathematical content which won't fit into the two-column measure easily.
  Selection of one-column output also affects the actions of other macros,
  particularly those controlling figures and tables.

\item {Referee} This selects referee mode (double spaced) if required
  (default = not selected). Figure captions and Tables are not double
  spaced by this option.

\item {authorcomment} This creates a catchline at the bottom of the page
  which authors may wish to use to keep track of the versions of their
  article.

\item {begintopmatter} This macro should be used just before defining the
  article title and author names.  If you omit this macro \TeX\ will
  complain loudly when it reaches the |\maketitle| macro.

\item {title} Set the article title, e.g.
\beginlines
|\title{Dust envelopes around RV Tauri stars}|
\endlines

\item {author} Set the article author(s), e.g.
\beginlines
|\author{A. V. Raveendran}|
\endlines

\item {affiliation} Set the author affiliation(s), e.g.
\beginlines
|\affiliation{Indian Institute of Astrophysics..}|
\endlines
Multiple author names should be set as follows.  Do not use
`\&' between names, always use `and'.  Each author name is
listed, followed by a reference mark (usually a superscripted
number).  The reference mark refers to each author's
respective affiliations in a list which follows afterwards.
For example,
\beginlines
\vbox{%
|\author{A.~Moorhouse,$^{1,2}$|
|        P.~W.~J.~L.~Brand,$^1$|
|        T.~R.~Geballe$^3$ and M.~G.~Burton$^4$}|
|\affiliation{$^1$ Department of Astronomy, ...}|
|\affiliation{$^2$ Present address: Dublin|
|                  Institute for ...}|
|\affiliation{$^3$ Joint Astronomy Centre ...}|
|\affiliation{$^4$ NASA Ames Research Center ...}|
}%
\endlines
Note that the `present address' in
the above example is treated as though it were an affiliation.  Similarly,
fellowships or other posts, for example `Visiting Observer, Mount John
University Observatory \dots' should be listed in the acknowledgments.

\item {shortauthor} Define the even-page running head.
\beginlines
|\shortauthor{R. A. Stathakis and E. M. Sadler}|
\endlines
Initials only should be used in running heads; use `and',
not~`\&', to separate the final two names.  When there is a
long list of authors (four or more) use the form
\beginlines
|\shortauthor{D.~T.~Wickramasinghe et al.}|
\endlines

\item {shorttitle} Define the odd-page running head.
\beginlines
|\shorttitle{The H\,{\eightit I} spectra}|
\endlines
Notice the use of the |\,| (thinspace) after the `H' in the above example.
The |\eightit| simulates the effect of an italic small-caps.
If you require roman (upright) text in the short-title, say for `IRAS',
you would use:
\beginlines
|\shorttitle{...{\rm IRAS}...}|
\endlines
It may also be necessary to add an italic correction |\/| before the |\rm|
to improve the spacing.

\item {abstract} Set the abstract information, e.g.
\beginlines
|\abstract {This is the text of the abstract ...}|
\endlines
This design macro requires that the text (which can be
longer than one paragraph) is enclosed in braces.
The abstract must fit on to the
first page of the article when typeset.

\item {keywords} Set any article key words,  e.g.
\beginlines
|\keywords {circumstellar matter|
|           -- infrared: stars.}|
\endlines
The same applies for |\keywords| as for the |\abstract| macro.

\item {maketitle} This macro must be used just before the first section
  or the first text paragraph.
\endexhang


\subsection{Headings}

Some headings are capitalized. Where this is true the design macro will
automatically capitalize whatever you key. As a rule, it is advisable to
capitalize the first letter, and any words that normally start with a capital,
i.e. proper nouns, abbreviations, but key all other words in lower case.

The |\section|, |\subsection| and |\subsubsection| mac\-ros are
automatically numbered. To produce unnumbered headings, `star' forms of
these macros exist, e.g. |\section*|.
%
\beginexhang{subsubsection}
\item {section} Start a new section, e.g.
\beginlines
|\section{Introduction}|
\endlines
For main section headings such as `Acknowledgments' and
`References' use the |\section*| macro, e.g.
\beginlines
|\section*{Acknowledgments}|
\endlines
The |\section| command is also used to produce appendices
(see Subsection~3.11 for more information).%%

\item {subsection} Start a new subsection, e.g.
\beginlines
|\subsection{Colour--colour diagram}|
\endlines

\item {subsubsection} Start a new subsubsection, e.g.
\beginlines
|\subsubsection{Correlation with subgroups}|
\endlines

\item {paragraph} Start a new subsubsubsection, e.g.
\beginlines
|\paragraph{Correlation with subgroups.} Text|
| runs on after heading...|
\endlines
It is important to note that text runs on after a
|\paragraph|. There should be no break between this heading
and the next paragraph.
\endexhang

\noindent The macro |\section| forces the text of the heading into upper
case, and |\subsection| emboldens the text.  When headings contain names
with lowercase or small capital letters, place these letters in the
argument of |\lowercase|, e.g.
\beginlines
|N\lowercase{a}\,{\sixbf I}/%|
|C\lowercase{a}\,{\sixbf II}|
\endlines
to get `\dots\ {\bf Na\,{\sixbf I}/Ca\,{\sixbf II}}\ \dots' in a section
heading. The |\sixbf| commands produce a simulated bold small-caps.
This technique can also be applied to the running heads; see the example in
|\shorttitle|.

The paragraph indent on any text following a |\section|, |\subsection|
or |\subsubsection| is automatically removed by the macros.


\subsection{Lists}
\subsubsection{Numbered lists}

Numbered lists are keyed in a simple and straightforward way. They begin
with a |\beginlist| command. Each item is marked with |\item| with its
number (in round braces) followed by the text for the item. The number
should be in lower case roman numerals. The list is ended with |\endlist|.
For example,
\beginlines
|\beginlist|
|\item (i) the attenuated and diluted stellar|
|  radiation;|
|\item (ii) scattered radiation, and|
|\item (iii) reradiation from other grains.|
|\endlist|
\endlines

\Notes

\beginlist
\item (i) Extra white space is automatically added above and below the list.
\item (ii) Outside the scope of the |\beginlist| and |\endlist| commands the
  |\item| command reverts to its plain \TeX\ definition. Don't use the
  plain \TeX\ |\item| command on its own, as the spacing and indents will
  be incorrect.
\item (iii) The paragraph indentation on the first paragraph following the
  |\endlist| command is removed automatically if you leave no blank
  line between the |\endlist| and the text.
\endlist


\subsubsection{Unnumbered lists}

These should be keyed in the same way as numbered lists (described above),
except that each item in the list has no number in round braces.


\subsection{Illustrations (or figures)}

Figures should be keyed as follows:
\beginlines
|\beginfigure{|{\em n\/}|}|
|  \vskip 3cm|
|  \caption{{\bf Figure |{\it f}|.} An example figure in|
|    which space has been left for the artwork.}|
|\endfigure|
\endlines
Figure captions should be below the figure itself, therefore
the |\caption| command should appear after the figure or space
left for an illustration.
The {\em n\/} value is the logical figure number. This number determines
the output order of the figure (in two-column mode).
It must start at~1 and increase with each successive figure.
\beginfigure{1}
  \vskip 3cm
  \caption{{\bf Figure 1.} An example figure in which space has been
    left for the artwork.}
\endfigure
The |\caption| macro is only valid in the scope of
|\beginfigure|$\ldots$|\endfigure|.

The example above will produce a single-column figure in two-column mode.
To produce a double-spanning figure use:
\beginlines
|\beginfigure*{|{\em n\/}|}|
|  |$\ldots$
|  \caption{|$\ldots$|}|
|\endfigure|
\endlines
Notice that |\beginfigure*| ends with |\endfigure|. If the text in the
caption is less than one line long it is centred automatically, otherwise
it is set full-out.

\Notes

\beginlist
\item (i) If there is more than one figure panel to a caption, the depth
  value should increase by 13pt (4.5mm) for every extra figure (if they are
  one above another). This allows for a gap between each figure panel.

\item (ii) If a figure occupies one complete page, insert a depth that does
  not completely fill the page, otherwise the figure may be output at the
  end of the paper (or not at all)!
\endlist

See `Instructions for Authors' in Monthly Notices for submission of
artwork.

\subsubsection{Points to note for figures in one-column articles}

\beginlist
\item (i) All figures (and their captions) will be set to full width even
  if they are keyed using |\beginfigure|$\ldots$|\endfigure|.
  Captions shorter than one line will be centred as normal.

\item (ii) The logical figure number is ignored in one-column mode.
  Therefore the figures are output in the order in which they appear in
  the source.

\item (iii) If a figure is placed very early in the source code,
  it is possible for it to float to the top of the first page
  (above the title). In this case, move the figure one paragraph down and
  try again. It may be necessary to do this with other figures to keep the
  output order correct.
\endlist


\subsection{Tables}

Tables should be keyed something like this:
\beginlines
|\begintable{|{\em n\/}|}|
|  \caption{{\bf Table |{\em t\/}|.} |$\ldots$|}|
|  \halign{| $<$alignment$>$ |}|
|  \tabletext{| text below table, table footnotes, etc. |}|
|\endtable|
\endlines
The {\em n\/} value is the logical table number, and {\em t\/} is the
table number. The logical table number determines the output order of the
table (in two-column mode).
It must start at~1 and increase with each successive table.

The table caption should appear before the body of the table.
The |\tabletext| macro is provided for table notes, and table footnotes.
It can contain more than one paragraph of text. Ten points of space are
automatically added above |\tabletext|. Only one |\tabletext| is allowed
per table. The usage of |\tabletext| is optional.

If you wish to insert non-aligned text into the body of the alignment do
not use |\noalign{|{\em text\/}|}| as this will make the table appear to
be full width to the macros, resulting in the table being set flush left.
In this case you can either use |\multispan| or use
|\noalign{\hbox{|{\em text\/}|}}|.

The caption, and any text below the table will be set to the table
width, when the table is centred by the macros.
The |\caption| and |\tabletext| macros are only valid in the scope of the
|\begintable|$\ldots$|\endtable|.

Table~1 is produced with the following code:
\beginlines
|\begintable{1}|
|  \caption{{\bf Table 1.} Radio-band beaming|
|    model parameters for FSRQs and BL Lacs.}|
|  \halign{#\hfil & \quad \hfil#\hfil\quad &|
|           \hfil#\hfil\quad & \hfil#\hfil\quad &|
|           \hfil#\hfil\quad & \hfil#\hfil\quad &|
|           \hfil#\hfil\cr|
|  Class   & $\gamma_1$ & $\gamma_2$ & $\langle|
|            \gamma \rangle$ & $G$ & $f$|
|          & $\theta_{\rm c}$ \cr|
|  BL Lacs & 5 & 36 & 7  & $-4.0$ & $1.0\times|
|    10^{-2}$ & 10$^\circ$ \cr|
|  FSRQs   & 5 & 40 & 11 & $-2.3$ & $0.5\times|
|    10^{-2}$ & 14$^\circ$ \cr|
|  }|
|  \tabletext{{\em G} is the slope of the Lorentz|
|    factor distribution, i.e. $n(\gamma)\propto|
|    \gamma^G$, extending between $\gamma_1$|
|    and $\gamma_2$, with mean value $\langle|
|    \gamma\rangle$, {\em f\/} is the ratio|
|    between the intrinsic jet luminosity and the|
|    extended, unbeamed luminosity, while|
|    $\theta_{{\rm c}}$ is the critical angle|
|    separating the beamed class from the parent|
|    population.}|
|\endtable|
\endlines

\begintable{1}
  \caption{{\bf Table 1.} Radio-band beaming model parameters
           for FSRQs and BL Lacs.}
  \halign{#\hfil&\quad \hfil#\hfil\quad& \hfil#\hfil\quad&
          \hfil#\hfil\quad& \hfil#\hfil\quad& \hfil#\hfil\quad&
          \hfil#\hfil\cr
  Class   & $\gamma_1$ & $\gamma_2$ & $\langle \gamma \rangle$ & $G$ & $f$
    & $\theta_{\rm c}$ \cr
  BL Lacs & 5 & 36 & 7  & $-4.0$ & $1.0\times 10^{-2}$ & 10$^\circ$ \cr
  FSRQs   & 5 & 40 & 11 & $-2.3$ & $0.5\times 10^{-2}$ & 14$^\circ$ \cr
  }
  \tabletext{{\em G} is the slope of the Lorentz factor distribution, i.e.
    $n(\gamma)\propto \gamma ^G$, extending between $\gamma _1$ and
    $\gamma_2$, with mean value $\langle \gamma \rangle$, {\em f\/} is the
    ratio between the intrinsic jet luminosity and the extended, unbeamed
    luminosity, while $\theta_{{\rm c}}$ is the critical angle separating
    the beamed class from the parent population.}
\endtable

\noindent The example above will produce a single-column table in two-column
mode. To produce a double-spanning table use:
\beginlines
|\begintable*{|{\em n\/}|}|
|  \caption{|$\ldots$|}|
|  \halign{|$\ldots$|}|
|  \tabletext{|$\ldots$|}|
|\endtable|
\endlines
Notice that |\begintable*| ends with |\endtable|.

Tables are allowed to have single horizontal rules, at the head
and foot only. Horizontal rules should have 3pt of space above and below
them. Vertical rules should not be used.

If a table occupies one complete page, you may find it necessary to reduce
its depth slightly, so that it doesn't completely fill the page, otherwise
the table may be output at the end of the paper (or not at all)!


\subsubsection{Points to note for tables in one-column articles}

\beginlist
\item (i) Tables that will fit into a column in two-column mode will be
  centred on the full page width in one-column mode.

\item (ii) The logical table number is ignored in two-column mode.
  Therefore the tables are output in the order in which they appear in
  the source.

\item (iii) If a table is placed very early in the source code,
  it is possible for it to float to the top of the first page
  (above the title). In this case, move the table one paragraph down and
  try again. It may be necessary to do this with other tables to keep the
  output order correct.
\endlist


\subsection{Captions for continued figures and tables}

If a very large figure or table does not fit on one page,
it must be split into two floats; the second float should use a
continued caption in the form:
\smallskip
\centerline{{\bf Figure 6} -- {\it continued}}
\smallskip
\noindent The figure or table number in the continued caption should be
the same as in the original caption. These captions should be keyed as
follows:
\beginlines
|\begintable{|{\it n\/}|}|
|  \caption{{\bf Table |{\it t\/}|} -- {\it continued}}|
|  :|
|\endtable|
\endlines
Notice that there is no full-point after the figure/table number.


\subsection{Landscape pages}

If a table or illustration is too wide to fit the standard measure, it
must be turned, with its caption, through 90 degrees anticlockwise. 
Landscape illustrations and/or tables cannot be produced directly
using the MN macros because \TeX\ itself cannot turn the
page, and not all device drivers provide such a facility.

The first step is to produce blank pages (with a running head) in the
output, so that the landscape material can be pasted in later. How
this is done depends on whether your article is in one or two columns.

For one-column articles use the following:
\beginlines
|\pageinsert|
|  \vfil\centerline{{\bf Figure |{\em f\/}|.} Landscape|
|    figure to go here.}\vfil|
|\endinsert|
\endlines
otherwise use
\beginlines
|\beginfigure*{|{\em n\/}|}|
|  \vbox to 646pt{\vfil \caption{{\bf Figure |{\em f\/}|.}|
|    Landscape figure to go here.}\vfil}|
|\endfigure|
\endlines
for two-column articles. You may find it necessary to move the above code
up or down the source code until the blank page appears on the page after
the first reference.

Next create a separate document containing the command |\landscape| near
the top (or use |mnland.tex| as a template).
In this file include the complete tables and illustrations (with captions)
using the figure and table macros provided, remembering to number the
captions in the correct sequence, e.g.
\ifCUPmtplainloaded \else \eject\fi %%
\beginlines
|\ifx\mnmacrosloaded\undefined \input mn\fi|
\smallskip
|% use the following if your driver supports it|
|% \special{landscape}|
\smallskip
|% you may require \pageoffset for landscape|
|% \pageoffset{0pc}{-1.5pc}|
\smallskip
|\landscape|
|\authorcomment{Landscape material to be pasted|
|  into the article.}|
\smallskip
|\begintopmatter|
|\maketitle|
\smallskip
|\beginfigure{1}|
|\caption{{\bf Figure 4.} Photometric|
|  comparisons |$\ldots$|}|
|\endfigure|
\smallskip
|:|
\smallskip
|\bye|
\endlines
Once you have successfully processed the new file with the MN macros, you
can pass the resulting output through your dvi printer driver. Because the
output of the MN macros is wider than it is deep, the page has to be printed
landscape on your output device.

Some dvi printer drivers will understand the `landscape' |\special| command
and will automatically rotate the output, while others need to be told from
the command line. Consult your local documentation if you don't know how to
do this.


\subsection{Plate pages}

These are provided for tip-in plates, and should only be used for
these. The plate page macros create a blank page with a special running
head; its contents can be set using the |\plate| command. The text in the 
head should be keyed as shown below. The {\em no\/} and {\em vol\/}
numbers will be determined by the typesetter.
\beginlines
|\beginplatepage|
|  \plate{Opposite p.~|{\em no\/}|, MNRAS, {\bf |{\em vol\/}|}}|
|  \caption{{\bf Figure |{\em f\/}|.} |$\ldots$|}|
|\endplatepage|
\endlines
If the plate is a `landscape' plate its caption (if any) should be set
using a separate `landscape' file (as described above). If the plate is
to be placed `portrait' its caption can be set by using the |\caption|
command as shown above. The style of the caption should be the same as for
normal figure captions. If the plate fills most of the page, it is advisable
to place the caption at the very bottom of the page -- this can be achieved
by using |\vfill| above the caption.

Plate pages will always appear on the page following the one on which the
|\endplatepage| command is encountered. At present it is impossible to have
two plate pages side by side, since there must be at least one page between
them. If a new plate page is started before a previous one is output the
first plate page is lost.


\subsection{Footnotes}

In the two-column format, footnotes should be keyed using |\note|, e.g.
\beginlines
|text\note {|{\em symbol\/}|}{|{\em footnote text}$\ldots$|} text|
\endlines
where {\em symbol\/} should be in the sequence:
$\star$ (|\star|), \dag, \ddag, \S, \P, $\|$, $\star\star$ (|\star\star|),
\dag\dag, \ddag\ddag, \S\S, \P\P, $\|\|$. 
The |\note| command should only be used for footnotes in the main text.

In the one-column format, footnotes should be keyed in the standard plain 
\TeX\ way using |\footnote|, e.g.
\beginlines
|text\footnote {|{\em symbol\/}|}{|{\em footnote text}$\ldots$|} text|
\endlines
where {\em symbol\/} should be in the above sequence.
Again, the |\footnote| command should only be used for footnotes in the main text.

\subsection{Bibliography}

References to published literature should be quoted in text by author
and date: e.g.\ Draine (1978) or (Begelman, Blandford \& Rees 1984).
Where more than one reference is cited having the same author(s) and date,
the letters a,b,c, $\ldots$ should follow the date: e.g.\ Smith (1988a),
Smith (1988b), etc. 


\subsubsection{References in the text}

References in the text are given by author and date, and, whichever
method is used to produce the bibliography, the references in the text
are done in the same way.
When you introduce a three-author paper, you should list all 
three authors at the first citation, and thereafter use et al.

\subsubsection{The list of references}

The following listing shows how references should be keyed in the style of
the journal.
\beginlines
|\section*{References}|
\smallskip
|\beginrefs|
|\bibitem Butcher J., 1992, Copy-editing:|
|    The Cambridge Handbook, 3rd edn.|
|    Cambridge Univ. Press, Cambridge|
|\bibitem The Chicago Manual of Style, 1982.|
|    Univ. Chicago Press, Chicago|
|\bibitem Blanco P., 1991, PhD thesis,|
|    Edinburgh University|
|\bibitem Brown A. B., Jones C. D., 1989,|
|    in Robinson E. F., Smith G. H., eds,|
|    Proc. IAU Symp. 345, Black Dwarfs.|
|    Kluwer, Dordrecht, p. 210|
|\bibitem Edelson R. A., 1987, ApJ, 313, 651|
|\bibitem Lamport L., 1986, \LaTeX: A Document|
|    Preparation System. Addison--Wesley,|
|    New York|
|\bibitem Mirabel I. F., Sanders D. B., 1989,|
|    ApJ, 340, L53|
|\bibitem Misner C. W., Thorne K. S.,|
|    Wheeler J. A., 1973, Gravitation.|
|    Freeman, San Francisco|
|\bibitem Sopp H. M., Alexander P., 1991,|
|    MNRAS, 251, 112|
|\bibitem Stella L., Campana S., 1991, in|
|    Treves A., Perola G. C., Stella L., eds,|
|    Iron Line Diagnostic in X-ray Sources.|
|    Springer--Verlag, Berlin, p. 230|
|\endrefs|
\endlines
The following rules apply for the ordering of your references:
\beginlist
\item (i) if an author has written several papers, some with other authors,
      the rule is that the single-author papers precede the two-author
      papers, which, in turn, precede the multi-author papers;
\item (ii) within the two-author paper citations, the order is determined
      by the second author's surname, regardless of date;
\item (iii) within the multi-author paper citations, the order is
      chronological, regardless of author surnames.
\endlist

\Notes

\beginlist
\item (i) The |\bibitem| command is undefined unless it is used in the
  scope of the |\beginrefs|$\ldots$|\endrefs|.
\item (ii) Bibliographical items can be longer than one paragraph.
\item (iii) The paragraph indentation on the first paragraph following the
  |\endrefs| command is removed automatically if you leave no blank
  line between the |\endrefs| and the text.
\endlist


\subsection{Appendices}

The appendices section of your article should start with a |\appendix|,
after which each |\section| starts a new appendix. For example,
\beginlines
|\appendix|
|\section{for authors}|
\endlines
will yield:\par
\smallskip
\centerline{\bf APPENDIX A:\enskip FOR AUTHORS}\par
\smallskip
\noindent The |\appendix| macro should only be used once.

If the appendix has no subtitle, the parameter to the |\section| command
should be left empty. For example,
\beginlines
|\section{}|
\endlines
will produce:\par
\smallskip
\centerline{\bf APPENDIX B}\par
\smallskip
\noindent Any subsections or subsubsections in the appendix are
automatically numbered.
You should also note that displayed equations in appendices should be
numbered (A1), (A2) for Appendix A, and (B1), (B2) for Appendix B, etc.

The numbering for displayed equations can be made automatic by using the
|\stepeq| macros described in Subsubsection~3.13.2.%%

Figures and Tables should also be numbered in a similar way,
e.g. Fig. A1, A2, Table A1, A2 in appendices.


\subsection{Typeface selection}

The normal plain \TeX\ typeface conventions apply. The following faces
are available as normal: |\rm|, |\it|, |\bf|, |\sl|, |\sf|, |\sc|,
|\tt|, |\mit|, |\cal| and |\oldstyle|.

Bold versions of |\cal| and |\oldstyle| can be produced in
combination with |\bmath|. Use of |\bmath| on its own will provide bold
math italic letters.

A new |\em| command provides {\em emphasis\/} for important words.
The |\em| command will automatically switch the face of the emphasized
words to make them stand out. So,
\beginlines
|\rm this is an {\em emphasized\/} word.|
|\it this is an {\em emphasized} word.|
\endlines
gives\par
\centerline{\rm  this is an {\em emphasized\/} word.}
\centerline{\it this is an {\em emphasized\/} word.}
\Half
\noindent Notice the use of the italic correction command (|\/|) in the
above example.

The following are fully loaded in text, script and scriptscript sizes:
|\rm|, |\bf|, math italic, math symbol, bold math italic and bold symbol.
The faces |\it|, |\sl|, |\tt|, |\sc| and |\sf| are loaded at text size only.
See |fonttest.tex| for a better idea of how these work.


\subsection{Typesetting mathematics}
\subsubsection{Displayed mathematics}

Equations should be keyed using normal plain \TeX\ macros.
Display mathematics are automatically set flush left by the macros.
The standard plain \TeX\ math commands |\eqalign|, |\eqalignno| will
work as before. The |\leqalignno| command is switched automatically
to |\eqalignno| to prevent the equation number from crashing into the
equation. If you wish to use |\displaylines|, this has to be handled
in a slightly different way. For example,
$$
\displaylines{%
  \hbox to \hsize{}\cr
  [\nu_1]-[\nu_2]=-2.5\log [f(\nu_1)/f(\nu_2)],\hfill\stepeq\cr
  \alpha=-(1+Q)\beta-3,\hfill\stepeq\cr
  q=2+\gamma -Q.\hfill\stepeq\cr}
$$
was produced with:
\beginlines
|$$|
|\displaylines{%|
|  \hbox to \hsize{}\cr|
|  [\nu_1]-[\nu_2]=-2.5\log [f(\nu_1)/f(\nu_2)],|
|    \hfill\stepeq\cr|
|  \alpha=-(1+Q)\beta-3,\hfill\stepeq\cr|
|  q=2+\gamma -Q.\hfill\stepeq\cr}|
|$$|
\endlines
Notice the |\hbox to \hsize{}| to ensure that the equation is set to the
full width. The |\hfill|'s ensure that the equations are set flush left
and the equation numbers are set flush right.

If the equations in |\displaylines| are unnumbered, you still need the
|\hfill|'s to ensure the equations are set flush left.


\subsubsection{Automatic equation numbering}

Displayed equations can be numbered automatically by the use of |\stepeq|.
For example,
\beginlines
|$$|
| \alpha=-(1+Q)\beta-3,\eqno\stepeq|
|$$|
\endlines
which produces:
$$
\alpha=-(1+Q)\beta-3,\eqno\stepeq
$$
The |\stepeq| macro can be used in any of the places where a equation
number is normally expected. Sub-equation numbering is also provided,
allowing equation numbers in the form (2a) to be produced. For example,
$$
\eqalignno{%
           \alpha & =-(1+Q)\beta-3, & \startsubeq\cr
                q & =2+\gamma -Q. & \stepsubeq\cr
  [\nu_1]-[\nu_2] & =-2.5\log [f(\nu_1)/f(\nu_2)] & \stepsubeq\cr}
$$
was produced by:
\ifCUPmtplainloaded \else \eject\fi %%
\beginlines
|$$|
|\eqalignno{%|
|  \alpha & =-(1+Q)\beta-3, & \startsubeq\cr|
|       q & =2+\gamma -Q.   & \stepsubeq\cr|
| [\nu_1]-[\nu_2] & =-2.5\log [f(\nu_1)/f(\nu_2)]|
|                 & \stepsubeq\cr}|
|$$|
\endlines
The sub-equation number is reset each time a |\stepeq| is used. Equation
numbering is automatically reset to `(A1)' when a |\appendix| is used.


\subsubsection{Bold math italic}

To obtain bold math italic, you should use |\bmath|.
So to obtain:
$$
  d(\bmath{s_{t_u}}) = \langle [RM(\bmath{X_y}
  + \bmath{s_t}) - RM(\bmath{x_y})]^2 \rangle
$$
you would key:
\beginlines
|$$|
|  d(\bmath{s_{t_u}}) = \langle [RM(\bmath{X_y}|
|  + \bmath{s_t}) - RM(\bmath{x_y})]^2 \rangle|
|$$|
\endlines
This facility is available in all typesizes.


\subsubsection{Bold Greek and other bold symbols}

Bold lowercase Greek characters can be obtained by prefixing
the normal (unbold) symbol name with a `b', e.g.\ |\bgamma| gives $\bgamma$.
This rule does not apply to bold |\eta|, as this would lead to a name
clash with |\beta|. Instead use |\boldeta| for bold eta. Note that there
is no |\omicron| (so there is no |\bomicron|), just use `o' in math mode
for omicron and `|\bmath{o}|' for bold omicron.

Bold versions of most of the other symbols in appendix~F in the \TeX book
can be obtained in the same way.

For bold uppercase Greek, prefix the unbold character name with |\bf|,
e.g.\ |\bf\Gamma| gives $\bf\Gamma$.
Upper and lowercase Greek characters are available in all typesizes.

You can then use these definitions in math mode, as you would normal Greek
characters:
%
\beginlines
|$$|
|  \balpha_{\bmu} = {\bf\Theta} \alpha.|
|$$|
\endlines
%
will produce
%
$$
  \balpha_{\bmu} = {\bf\Theta} \alpha.
$$
To save \TeX's valuable memory the symbol names for the bold math
characters are not loaded automatically. To load them simply type
\beginlines
|  \loadboldmathnames|
\endlines
in the document. Alternatively, if you only need one or two of them,
simply copy the appropriate definitions from |mn.tex|
to your document. For a complete list of the bold math symbols
supplied, see the file |mn.tex|.


\subsubsection{Upright Greek characters}

You can obtain upright Greek characters if you have access to the
American Maths Society Euler fonts (version 2.0), but you may not
have these. In this case, you will have to use the normal math italic
symbols and the typesetter will substitute the corresponding upright
characters. You will make this easier if you can use the macros |\upi|,
|\umu| and |\upartial| etc.\ in your text to indicate the need for upright
characters, together with the following definitions in the preamble
(before |\begintopmatter|):

\subsubsection*{Authors with AMS fonts}

\beginlines
|\ifCUPmtplainloaded \else|
|  \NewSymbolFont{upmath} {eurm10}|
|  \NewMathSymbol{\upi}     {0}{upmath}{19}|
|  \NewMathSymbol{\umu}     {0}{upmath}{16}|
|  \NewMathSymbol{\upartial}{0}{upmath}{40}|
|\fi|
\endlines

\subsubsection*{Authors without AMS fonts}

\beginlines
|\ifCUPmtplainloaded \else|
|  \def\umu{\mu}|
|  \def\upi{\pi}|
|  \def\upartial{\partial}|
|\fi|
\endlines
Wether you have AMS fonts or not, the |\if..| and |\fi| are required in the
above examples to ensure that when your article is typeset in Monotype
Times, the correct definitions for these symbols are used.

The sample pages, guide and fonttest can be made to use AMS fonts if you
have them. To use them, just uncomment the following line in the preamble
of |mnguide.tex|, |mnsample.tex| and |fonttest.tex|:
%
\beginlines
|%\AMStwofontstrue|
\endlines
%
If you do this, the following upright symbols are used in the
sample pages, guide and fonttest: |\upi|, |\umu| and |\upartial|.


\subsubsection{Special symbols}

The macros for the special symbols in Tables~2 and~3 have been taken from
the Springer Verlag `Astronomy and Astrophysics' design, with their
permission. They are directly compatible and use the same macro names.
These symbols will work in all text sizes, but are only guaranteed to work
in text and displaystyles. Some of the symbols will not get any smaller
when they are used in sub- or superscripts, and will therefore be displayed
at the wrong size. Don't worry about this as the typesetter will be able to
sort it out.
%
\begintable*{2}
\caption{{\bf Table 2.} Special symbols which can only be used in
math mode.}
\advance\baselineskip by 2pt
\halign{#\hfil\quad&#\hfil\quad&#\hfil\qquad\qquad
        &#\hfil\quad&#\hfil\quad&#\hfil\cr
Input & Explanation & Output & Input & Explanation & Output\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
|\la|     & less or approx       & $\la$     &
  |\ga|     & greater or approx    & $\ga$\cr
|\getsto| & gets over to         & $\getsto$ &
  |\cor|    & corresponds to       & $\cor$\cr
|\lid|    & less or equal        & $\lid$    &
  |\gid|    & greater or equal     & $\gid$\cr
|\sol|    & similar over less    & $\sol$    &
  |\sog|    & similar over greater & $\sog$\cr
|\lse|    & less over simeq      & $\lse$    &
  |\gse|    & greater over simeq   & $\gse$\cr
|\grole|  & greater over less    & $\grole$  &
  |\leogr|  & less over greater    & $\leogr$\cr
|\loa|    & less over approx     & $\loa$    &
  |\goa|    & greater over approx  & $\goa$\cr
|\bbbr| & Blackboard bold R & $\bbbr$ &
  |\bbbm|   & Blackboard bold M & $\bbbm$ \cr
|\bbbn| & Blackboard bold N & $\bbbn$ &
  |\bbbf|   & Blackboard bold F & $\bbbf$ \cr
|\bbbh| & Blackboard bold H & $\bbbh$ &
  |\bbbk|   & Blackboard bold K & $\bbbk$ \cr
|\bbbp| & Blackboard bold P & $\bbbp$ &
  |\bbbone| & Blackboard bold 1 & $\bbbone$ \cr
|\bbbc| & Blackboard bold C & $\bbbc$ &
  |\bbbq|   & Blackboard bold Q & $\bbbq$ \cr
|\bbbt| & Blackboard bold T & $\bbbt$ &
  |\bbbs|   & Blackboard bold S & $\bbbs$ \cr
|\bbbz| & Blackboard bold Z & $\bbbz$ \cr
%
\noalign{\vskip 3pt\hrule}
}
\endtable

\begintable*{3}
\caption{{\bf Table 3.} Special symbols which don't have to be
used in math mode.}
\advance\baselineskip by 2pt
\halign{#\hfil\quad&#\hfil\quad&#\hfil\qquad\qquad
        &#\hfil\quad&#\hfil\quad&#\hfil\cr
Input & Explanation & Output & Input & Explanation & Output\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
|\sun|      & sun symbol            & $\sun$     &
  |\degr|     & degree                & $\degr$\cr
|\diameter| & diameter              & \diameter  &
  |\sq|       & square                & $\sq$\cr
|\fd|       & fraction of day       & \fd        &
  |\fh|       & fraction of hour      & \fh\cr
|\fm|       & fraction of minute    & \fm        &
  |\fs|       & fraction of second    & \fs\cr
|\fdg|      & fraction of degree    & \fdg       &
  |\fp|       & fraction of period    & \fp\cr
|\farcs|    & fraction of arcsecond & \farcs     &
  |\farcm|    & fraction of arcmin    & \farcm\cr
|\arcsec|   & arcsecond             & \arcsec    &
  |\arcmin|   & arcminute             & \arcmin\cr
\noalign{\vskip 3pt\hrule}
}
\endtable

\ifCUPmtplainloaded
\subsubsection{Extra features in the Monotype Times version}

This section of the guide will only be included if the guide is \TeX ed
with the Times version of the MN macros (mtmn.tex). The following features
are only available in the Times version:
\beginlist
\item (i) All of the type sizes available are fully loaded.
\item (ii) Most of the symbols in Table~2 will be substituted
  with symbols from the |mtxm| font. Only |\sq| is substituted in Table~3.
\item (iii) All of the symbols in the |mtxm| and |mtym| fonts can be used,
  at any size (using the normal AMS names).
  If the author has used |mssymb.tex| then this can be removed, as most
  of this file is now included in MN. If the author has used the new AMS
  symbol fonts |msam| and |msbm| -- check the log file for missing
  characters (once you've removed |msam| and |msbm|).
  You have to do this because |msam| and |msbm| contain a few extra
  characters NOT in |mtxm| and |mtym|. If you find missing characters get
  help!
\item (iv) Uppercase blackboard bold is available in all sizes. e.g.
  \beginlines
  |$\Bbb{A}\ldots\Bbb{Z}$|\qquad gives\qquad $\Bbb{A}\ldots\Bbb{Z}$
  \endlines
  If the author has made-up their own uppercase blackboard bold characters
  you can safely use |\Bbb| instead.
\item (v) If the author has used the simulated Blackboard bold symbols
  these are automatically substituted for the real characters, except for
  |\bbbone| which is redefined to work better with Times fonts.
\endlist
\fi

\section{Example of section heading with
  S{\sevenbf MALL} C{\sevenbf APS},
  \lowercase{lowercase}, \textbfit{italic}, and bold
  Greek such as $\bmu^{\bkappa}$}

The above heading was produced with:
\beginlines
|\section{Example of section heading with|
|  S{\sevenbf MALL} C{\sevenbf APS},|
|  \lowercase{lowercase}, \textbfit{italic},|
|  and bold Greek such as $\bmu^{\bkappa}$}|
\endlines

\appendix
\section{for authors}

Table~A1 is a list of design macros which are unique to |mn.tex|. The list
displays each macro's name and description.
%
\begintable*{4}
\caption{{\bf Table A1.} Authors' notes.}
\vbox to 630pt{%
\halign{#\hfil&\quad #\hfil\cr
Macro name and syntax        & Description\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
|\pageoffset {h-off}{v-off}| & Adjust positioning of text area on paper.\cr
|\Referee|                   & Enable double-spaced referee mode.\cr
|\onecolumn|                 & Enable one-column mode (default =
                               two-column).\cr
|\landscape| & Enable landscape mode (default = portrait).\cr
             & The |\landscape| command automatically calls |\onecolumn|.\cr
|\loadboldmathnames|  & Enable the use of bold symbols, e.g. |\bgamma|\cr
|\authorcomment|             & Catchline for draft version/date.\cr
\noalign{\Half}
|\begintopmatter|            & Start the two-spanning topmatter.\cr
|\title {<text>}|            & Article title.\cr
|\author {<text>}|           & Author(s).\cr
|\affiliation {<text>}|      & Author affiliation(s).\cr
|\shortauthor {<text>}|      & Set the even-page running head.\cr
|\shorttitle {<text>}|       & Set the odd-page running head.\cr
|\abstract {<text>}|         & Abstract.\cr
|\keywords {<text>}|         & Key words.\cr
|\maketitle|                 & End the two-spanning topmatter.\cr
\noalign{\Half}
|\section {<text>}|          & Heading level A.\cr
|\section* {<text>}|         & Unnumbered A-heading.\cr
|\subsection {<text>}|       & Heading level B.\cr
|\subsubsection {<text>}|    & Heading level C.\cr
|\paragraph {<text>}|        & Heading level D.\cr
|\appendix|                  & Start the articles appendix section.
                               The |\section| command starts\cr
                             & a new appendix.\cr
\noalign{\Half}
|\stepeq|, |\startsubeq|, |\stepsubeq| & Automatic equation numbering.\cr
\noalign{\Half}
|\beginlist|                 & Numbered list:\cr
|  \item (i) <text>|         & Omit the number and round braces from
                               each |\item| for an unnumbered list.\cr
|  \item (ii) <text>|\cr
\noalign{\vskip-.25\baselineskip}
|   |$\ldots$\cr
\noalign{\vskip-.2\baselineskip}
|\endlist|\cr
\noalign{\Half}
|\beginrefs|                  & Bibliography.\cr
|  \bibitem <text>|\cr
\noalign{\vskip-.25\baselineskip}
|   |$\ldots$\cr
\noalign{\vskip-.2\baselineskip}
|\endrefs|\cr
\noalign{\Half}
|\beginfigure{n}|                          & Figures:\cr
|  <figure space>|            & Use the |\beginfigure*| form for a
                                double-spanning figure\cr
|  \caption{{\bf Figure n.} caption}|      & in two-column mode.\cr
|\endfigure|\cr
\noalign{\Half}
|\begintable{n}|                           & Tables:\cr
|  \caption{{\bf Table n.} caption}|
            & Use the |\begintable*| form for a double-spanning table\cr
|  <alignment>|                            & in two-column mode.\cr
|  \tabletext{<text>}|\cr
|\endtable|\cr
\noalign{\Half}
|\caption{{\bf Figure n} -- {\it continued}}| & Continued captions.\cr
|\caption{{\bf Table n} -- {\it continued}}|\cr
\noalign{\Half}
|\beginplatepage| & Plate pages.\cr
|  \plate{Opposite p.\ n, MNRAS, {\bf n}}|\cr
|  <figure space>|\cr
|  \caption{{\bf Figure n.} caption}|\cr
|\endplatepage|\cr
\noalign{\Half}
|\note|                     & Use for footnotes in two-column mode.\cr
\noalign{\Half}
|\Two, \OneHalf, \One, \Half| & Extra vertical space: These macros insert
                                white space, in multiples\cr
    & of the linefeed, between paragraphs. Use during page make-up in \cr
    & preference to plain \TeX's |\smallskip|, |\medskip| and |\bigskip|.\cr
\noalign{\Half}
|\bmath{math text}|, |\em| & Bold math and emphasized text.\cr
|\textbfit{text}|, |\mathbfit{text}| & Bold text italic (defined in
                                       the preamble of |mnsample.tex|).\cr
|\textbfss{text}|, |\mathbfss{text}|& Bold text sans serif (defined in
                                       the preamble of |mnsample.tex|).\cr
|\umu|, |\upi|, |\upartial| & Upright math characters. These will only
                              appear upright if you have\cr
                            & AMS v2.0 fonts. See ``upright greek
                              characters" for further information.\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
}}
\endtable


\section{for editors}

The additional features shown in Table~B1 may be used for production
purposes only.
%
\begintable*{5}
\caption{{\bf Table B1.} Editors' notes.}
\halign{#\hfil&\quad #\hfil\cr
Macro name and syntax  & Description\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
|\pageno=000|          & to set pagination; default = 1.\cr
|\pagerange{000--000}| & note the use of the en-rule\cr
|\letters|             & for short communications (adds L to folios)\cr
|\pagerange{L00--L00}| & for short communications\cr
|\microfiche{MN000/0}| & for articles accompanied by microfiche\cr
|\pubyear{0000}|       & catchline date\cr
|\volume{000}|         & catchline volume\cr
|\acceptedline{text}|  & acceptance date\cr
|\nofloat|             & Position a figure or table at the current position
                         (one-column only).\cr
  & The |\nofloat| macro should be positioned directly after the\cr
  & |\beginfigure|/|table|, and will cause the macros to use |\midinsert|\cr
  & (remember that |\midinsert| will turn into a |\topinsert| if there\cr
  & is not enough space).\cr
\noalign{\vskip 3pt\hrule\vskip 3pt}
}
\endtable


\section{Monthly Notices journal style}
        
Authors  submitting  \TeX\ or \LaTeX\ papers to Monthly  Notices  
may wish to note the following points regarding journal style. 
Adherence to correct style from the start will obviously save time
and effort later on, in terms of fewer requested subeditorial 
corrections.  The notes given here relate to common style errors found 
in Monthly Notices manuscripts, and are {\it not\/} intended to  be  
exhaustive. Please see the editorials in issues 257/2 and 260/1, as 
well as any recent issue of the journal, for more details. As far 
as  possible, the subeditor will indicate which of  your  changes 
would be best done globally, thus saving you time.
        
\subsection{Punctuation}

When deciding where to add commas, it may be helpful to read 
 through the sentence and note where the natural `pauses' occur.
The needs of readers for whom English is not a first language 
should be borne in mind when punctuating long sentences.
\ifCUPmtplainloaded \else \vadjust{\eject}\fi %%
For example, consider the following sentence as it
appeared in Monthly Notices:
`When we do not limit ourselves by constraints arising 
from the choice of an initial fluctuation spectrum, structures in 
an open universe, including the peculiar velocity structure, can 
be reproduced in a flat Lema\^{\i}tre universe for a large part of 
their evolution.' Now consider the same sentence without commas: 
`When we do not limit ourselves by constraints arising
from the choice of an initial fluctuation spectrum structures in
an open universe including the peculiar velocity structure can be
reproduced in a flat Lema\^{\i}tre universe for a large part of their
evolution.'


\subsection{Spelling}

Please  use British spelling -- e.g.\ centre not center,  labelled 
not  labeled. The following style regarding -ise and -ize  spellings  is
followed.  -ise: devise,  surprise,  comprise,  revise, 
exercise,  analyse. -ize: recognize, criticize, minimize,  emphasize, organize.

        
\subsection{Titles and section/subsection headings}

With the exception of section headings (e.g.\
{\bf INTRO\-DUC\-TION}$\ldots$),
capital letters should be used only where they occur in a normal
sentence -- e.g.\ 
`\textbfit{ROSAT\/} {\bf observations of the unusual star}$\ldots$', not
`\textbfit{ROSAT\/} {\bf Observations of the Unusual Star}$\ldots$'.

\subsection{Key words}

The  list of Monthly Notices key words is published with the  4th 
issue  of each volume. No other key words should be used.  Please 
use the correct layout for key words: 
\smallskip        

\noindent {\bf Key words:} galaxies: active -- galaxies: Seyfert -- 
radio continuum: galaxies.
        
\subsection{Hyphens and N-rules}

\beginlist
\item (i) Hyphens (one dash in \TeX/\LaTeX). Monthly Notices uses hyphens 
for compound adjectives (e.g.\ low-density gas, least-squares fit, 
two-component  model).  This also applies to simple  units  (e.g.\ 
1.5-m  telescope,  284.5-nm line), but not to  complex  units  or 
ranges,  which could become cumbersome (e.g.\ 15 km  s$^{-1}$  feature, 
100--200 $\umu$m observations).

\item (ii) N-rules (two dashes in \TeX/\LaTeX). These are used  (a)  to 
separate  key  words, (b) as parentheses (e.g.\  `the  results  -- 
assuming no temperature gradient -- are indicative of$\ldots$), (c) to 
denote a range (e.g.\ 1.6--2.2 $\umu$m), and (d) to denote the  joining 
of   two  words  (e.g.\  Kolmogorov--Smirnov  test,   Herbig--Haro 
object).
        
\item (iii) The  M-rule (three dashes in \TeX/\LaTeX) is not used in
Monthly Notices.
\endlist

        
\subsection{References}

It is important to use the correct reference style,  details  of 
which  can be found in the editorials cited above, and  which  is 
demonstrated in any recent issue of the journal. The main  points 
are summarized below.
%        
\beginlist
\item (i) In text -- for three-author papers, give all three  authors 
at first mention, and `et al.' thereafter.

\item (ii) In references list -- no bold or italic, no  commas  after 
author surnames, and no ampersand between final two author names.
Use  simplified abbreviations for frequently used journals  (e.g.\ 
MNRAS,  ApJ,  A\&A, PASP -- see full list in  editorial  in  issue 
260/1). List all authors if eight or less, otherwise `et al.' For 
example,
\endlist

\beginrefs
\bibitem Biggs J.D., Lyne A.G., 1992, MNRAS, 254, 257

\bibitem Brown A.B., Jones C.D., 1989, in Robinson E.F.,
Smith G.H.,  eds, Proc. IAU Symp. 345, Black Dwarfs. Kluwer, Dordrecht,
p.~210

\bibitem Felsteiner  J.,  Opher  R., 1991, in Treves A.,  ed.,
Iron  Line Diagnostics in X-ray Sources. Springer-Verlag, Berlin, p.~209

\bibitem Gunn  J.E., Knapp G., 1993, in Soifer B.T., ed., ASP
Conf.\ Ser.\ Vol.~43, Sky Surveys. Astron.\ Soc.\ Pac., San Francisco,
p.~267

\bibitem Peebles P.J.E., 1980, The Large-Scale Structure of the  Universe. Princeton Univ. Press, Princeton, NJ

\bibitem Pounds K.A. et al., 1993, MNRAS, 260, 77

\bibitem Williams B.G., 1992, PhD thesis, Univ.\ Edinburgh
\endrefs


\subsection{Maths}

Scalar  variables are italic; vectors are bold  italic;  matrices 
are  `bold Univers' font (like bold sans serif). Differential  d, 
complex  i, exponential e, sin, cos, tan, log, etc.,  are  roman. 
Sub/superscripts  that are physical variables are  italic,  while 
those  that are just labels are roman (e.g.\ $C_p$, but $T_{{\rm eff}}$).
Equations should be punctuated as part of the sentence.


\subsection{Miscellaneous}

e.g., i.e., cf., etc., are roman.
Single quotes `  ' not double quotes `` ".
Take care to use correct units -- see recent \hbox{issues} for  details. 
Use  superscript $-1$, not solidus /, for units -- e.g.\ km~s$^{-1}$ not 
km/s. The unit of arcseconds is arcsec when used to denote  angular  
size  or separation (e.g.\ `beamsize 12~arcsec',  `30~arcsec 
west  of  the star'); use \arcsec\ for positions (e.g.\  
Dec.~$-30^\circ$~29\arcmin~23\arcsec) (similarly for arcminutes). 
The unit of magnitudes is  mag, 
not superscript m. Percentages should be written `per cent',  not 
\%. Use the degree symbol $^\circ$ (|$^\circ$|)  except to denote, e.g., areas,  where      
`deg$^2$'  may be more appropriate (e.g.\ `a survey area of 3~deg$^2$').
Degree symbols should be positioned above the decimal  point  if 
there  is one -- i.e.\ 23\fdg 4 not 23.4$^\circ$ (similarly for
\ifCUPmtplainloaded \vadjust{\eject}\else\fi %%
superscript 
h, m, s, and \arcmin, \arcsec\ symbols in coordinates). See guide for coding.
Ionized  species  should be denoted by small caps,  with  a  thin 
space -- e.g.\ \hbox{He\,{\sc ii}}, \hbox{C\,{\sc iv}}, 
\hbox{[Fe\,{\sc ii}]} 465.8 nm, \hbox{N\,{\sc iii}} 463.4~nm.  If 
lack  of the correct font at your site prevents this from  coming 
out on your printout, it would be helpful if you were to indicate 
as such on your manuscript so that the subeditor knows that there 
is no need for correction.
Computer software (e.g.\ {\sc figaro}) should be in small capitals.
Satellite names should be italic (e.g.\ {\it Ginga, IRAS\/}).
The correct bracket order is $\{[( )]\}$.


\section{Trouble-shooting}

Authors may from time to time encounter problems with the  preparation  
of their papers in \TeX/\LaTeX. The appropriate  action  to 
take will depend on the nature of the problem -- the following is 
intended to act as a guide.
%
\beginlist
\item (i) If a problem is with \TeX/\LaTeX\ itself, rather than with the 
actual macros, \ifCUPmtplainloaded \else \vadjust{\eject}\fi %%
please refer to the appropriate handbooks for 
initial advice.\footnote{\dag}{\TeX : Knuth D., 1986, The \TeX book. 
Addison Wesley; \LaTeX: Lamport L., 1985, \LaTeX\ User's Guide and 
Reference Manual. Addison Wesley.} If the 
solution cannot be found, and you suspect that the problem lies 
with the macros, then please contact the RAS Journal Production
team at Blackwell Science (BS), 23 Ainslie
Place, Edinburgh EH3 6AJ, UK (Tel: 031 226 7232; Fax: 031 226 3803;
omit the first zero if calling from outside the UK).
The BS office will shortly be
accessible by email -- please see the Instructions for Authors on 
the inside back cover of Monthly Notices for details. Please 
provide precise details of the problem (what you were trying to 
do -- ideally, include examples of source code as well -- and 
what exactly happened; what error message was received).
        
\item (ii) Problems with page make-up, particularly in the two-column 
mode (e.g.\ large spaces between paragraphs, or under headings or 
figures; uneven columns; figures/tables appearing out of order). 
Please do {\it not\/} attempt to remedy these yourself using `hard' page 
make-up commands -- the typesetters at Cambridge University Press 
(CUP) will sort out problems when typesetting. (You may, if you 
wish, draw attention to particular problems when submitting the 
final version of your paper.)
        
\item (iii) If a required font is not available at your site, allow \TeX\
to substitute the font and report the problem on your disk 
documentation form. 
\endlist


\subsection{Fixes for coding problems}

The new versions of the style files and macros have been designed
to minimize the need for user-defined macros to create special
symbols. Authors are urged, wherever possible, to use the following
coding rather than create their own. This will minimize the
danger of author-defined macros being accidentally `over-ridden'
when the paper is typeset in Monotype Times (see Subsection~3.13, %%
`Typesetting mathematics').
%
\beginlist
\item (i) Fonts in sections and paper titles. The following are  examples
of styles that sometimes prove difficult to code.
\endlist


\subsection*{\it P\lowercase{aper titles}}

\boxit{\multi\seventeenpoint\bf
  A survey of \textbfit{IRAS\/} galaxies\\
  at $\bmath{\delta > {\bf 50}^\circ}$\endmulti}
%
is produced by:
%
\beginlines
|\title{A survey of \textbfit{IRAS\/} galaxies|
| \hfil\break at $\bmath{\delta>{\bf 50}^\circ}$}|
\smallskip
|\shorttitle{A survey of IRAS galaxies at $\delta|
|  > 50^\circ$}|
\endlines
\bigskip

\boxit{\multi\seventeenpoint\bf\noindent
  Observations of compact\\
  H\,{\elevenbf II} regions\endmulti}
%
is produced by:
%
\beginlines
|\title{Observations of compact|
|  H\,{\elevenbf II} regions}|
\smallskip
|\shorttitle{Observations of compact|
|  H\,{\eightit II} regions}|
\endlines


\subsection*{\it S\lowercase{ection headings}}

\boxit{\bf 1\quad THE \textbfit{IRAS\/} DATA FOR
  $\bmath{\delta > {\bf 50}^\circ}$}
%
is produced by:
%
\beginlines
|\section{The \textbfit{IRAS\/} data for|
|  $\bmath{\delta>{\bf 50}^\circ}$}|
\endlines
\bigskip

\boxit{\bf 2\quad H\,{\sevenbf II} GALAXIES AT
  $\bmath{\lowercase{z} > {\bf 1.6}}$}
%
is produced by:
%
\beginlines
|\section{H\,{\sevenbf II} galaxies at|
|  $\bmath{\lowercase{z}>{\bf 1.6}}$}|
\endlines


\subsection*{\it S\lowercase{ubsection headings}}
        
\boxit{\multi\bf 2.1\quad The \textbfit{IRAS\/} data for
  $\bmath{\delta > {\bf 50}^\circ}$: galaxies\\
  at $\bmath{z > {\bf 1.5}}$\endmulti}
%
is produced by:
%
\beginlines
|\subsection{The \textbfit{IRAS\/} data for|
|  $\bmath{\delta > {\bf 50}^\circ}$: galaxies|
|  \hfil\break at $\bmath{z > {\bf 1.5}}$}|
\endlines
\bigskip

\boxit{\bf 2.2\quad Observations of compact H\,{\sevenbf II} regions}
%
is produced by:
%
\beginlines
|\subsection{Observations of compact|
|  H\,{\sevenbf II} regions}|
\endlines
\bigskip

\boxit{\it 2.2.1\quad A survey of radio galaxies
  for $\delta > {\it 50}^\circ$}
%
is produced by:
%
\beginlines
|\subsubsection{A survey of radio galaxies|
|  for $\delta > {\it 50}^\circ$}|
\endlines
\bigskip
        
\boxit{\it 2.2.2\quad Determination of T$_{eff}$ in compact
  H\,{\sevenit II} regions}
%
is produced by:
%
\beginlines
|\subsubsection{Determination of T$_{eff}$ in|
|  compact H\,{\sevenit II} regions}|
\endlines

\beginlist
\item (ii) Small capitals and other unusual fonts in table and figure
captions:
\par\smallskip
\boxit{\eightpoint {\bf Figure 1.} Profiles of the H$\alpha$ and
  N\,{\sc iii} lines observed.}
%
is produced by:
%
\beginlines
|\caption{Profiles of the H$\alpha$ and|
|  N\,{\sc iii} lines observed.}|
\endlines
        
\item (iii) Multiple author lists (to get the correct vertical spacing 
and wraparound on the title page of a multiple-author paper).
\par\smallskip

\boxit{\multi
  \seventeenpoint\bf\noindent
  The variation in the\\
  strength of low-$\bmath{l}$ solar\\
  $\bmath{p}$-modes: 1981--2
  \medskip
  \fourteenpoint\noindent
  Y. Elsworth, R. Howe, G.R. Isaac,\\
  C.P. McLeod, B.A. Miller, R. New,\\
  C.C. Speake and S.J. Wheeler\endmulti
}
%
is produced by:
%
\beginlines
|\title{The variation in the\hfil\break|
|  strength of low-$\bmath{l}$ solar\hfil\break|
|  $\bmath{p}$-modes: 1981--2}|
\smallskip
|\shorttitle{The variation in the strength of|
|  low-$l$ solar $p$-modes: 1981--2}|
\smallskip
|\author{Y. Elsworth, R. Howe, G.R. Isaac,|
|  \hfil\break C.P. McLeod, B.A. Miller, R. New,|
|  \hfil\break C.C. Speake and S.J. Wheeler}|
\smallskip
|\shortauthor{Y. Elsworth et al.}|
\endlines
        
\item (iv) Ionized species (as used in the examples above). The correct 
style calls for the use of small capitals and a thin space after 
the symbol for the element: e.g.\ for \hbox{H\,{\sc ii}}, use the code 
|\hbox{H\,{\sc ii}}|. The use of the |\hbox| will stop the 
H and the {\sc ii} being separated.

\item (v) Lower case greek pi ($\pi$), mu ($\mu$) and partial ($\partial$).
In certain circumstances, the Monthly Notices style calls for these to be
roman [when pi is used to denote the constant 3.1415$\ldots$, mu is
used to denote `micro' in a unit (e.g.\ $\umu$m, $\umu$Jy), and partial
is a differential symbol]. See Subsubsection~3.13.5 for instructions.

\item (vi) Decimal degrees, arcmin, arcsec, hours, minutes and seconds. 
The symbol needs to be placed vertically above the decimal point. 
For example, the sentence
%
\beginquote
The observations were made along position angle
120\fdg 5, starting from the central coordinates
${\rm RA}(1950)=19^{\rm h}~22^{\rm m}~18\fs 2$,
${\rm Dec.}~(1950)=45^\circ~18'~36\farcs 4$
\endquote
%
uses the following coding:
%
\beginlines
|The observations were made along position angle|
|120\fdg 5, starting from the central coordinates|
|${\rm RA}(1950)=19^{\rm h}~22^{\rm m}~18\fs 2$,|
|${\rm Dec.}~(1950)=45^\circ~18'~36\farcs 4$|
\endlines

\item (vii) The correct coding for the prime symbol \arcmin\ is 
|\arcmin|, and that for \arcsec\ is |\arcsec|; see the two
tables on special symbols.
        
\item (viii) N-rules, hyphens and minus signs (see style guide for  
correct usage). To create the correct symbols in the sentence
%
\beginquote
The high-resolution observations were made along a
line at an angle of $-15^\circ$ (east from north)
from the axis of the jet, which runs north--south
\endquote
%
you would use the following code:
%
\beginlines
|The high-resolution observations were made along|
|a line at an angle of $-15^\circ$ (east from|
|north) from the axis of the jet, which runs|
|north--south|
\endlines

\item (ix) Vectors and matrices should be bold italic and bold sans
serif respectively. To create the correct fonts for the vector $\bmath{x}$
and the matrix \textbfss{P}, you should use |$\bmath{x}$| and
|\textbfss{P}| respectively; |\mathbfss| is for use in
math mode. Bold face text italic can be obtained by using
|\textbfit{..}| and |\mathbfit{..}| for math mode.
\ifCUPmtplainloaded \else \vfil\eject\fi %%
\item (x) Bold italic superscripts and subscripts. To get these
to come out in the correct font and the right size, you need to use
|\bmath|. You can create the output $\bmath{k_x}$ by typing |$\bmath{k_x}$|.
Try to avoid using \TeX\ commands to determine script sizes that are
already  defined in the macros. For example, macros such as
%
\beginlines
|\def\th{^\hbox{\sevenrm th}}|
\endlines
%        
are generating extra work;
%
\beginlines
|\def\th{^{\rm th}}|
\endlines
%
will do, and will get the size of the superscript right whether in main
text, tables or captions (the use of |\sevenrm| over-rides the macros).
Also, the |\hbox| is not necessary, as \TeX\ won't split a
superscript/subscript from its variable at a line break.

\item (xi) Calligraphic letters (uppercase only).
%
Normal uppercase calligraphic can be produced with |\cal| as
normal (in math mode). Bold calligraphic can be produced with |\bmath|,
e.g.\ |$\bmath{\cal A}$| gives $\bmath{\cal A}$.

\item (xii) Automatic scaling of brackets. The codes |\left| and  
|\right| should  be used to scale brackets automatically to
fit the equation being set. For example, to get
$$
  v = x \left( {N+2}\over {N} \right)
$$        
use the code
%
\beginlines
|$$|
|  v = x \left( {N+2}\over {N} \right)|
|$$|
\endlines
        
\item (xiii) Roman font in equations. It is often necessary to make some 
symbols roman in an equation (e.g.\ units, subscripts). For  example, 
to get the following output:
$$
  \sigma \simeq (r/13~h^{-1}~{\rm Mpc})^{-0.9},
  \qquad \omega = {{N-N_{\rm s}}\over {N_{\rm R}}},
$$
you should use:
%
\beginlines
|$$|
|  \sigma\simeq (r/13~h^{-1}~{\rm Mpc})^{-0.9},|
|  \qquad\omega={{N-N_{\rm s}}\over {N_{\rm R}}},|
|$$|
\endlines

\item (xiv) Continuation figure and table captions.
See Subsection~3.6. %%
\endlist


\subsection{Springer-Verlag macro names}

These have been incorporated from the Astronomy \& Astrophysics \LaTeX\ 
style file, to aid in the creation of various commonly used
astronomical symbols. Please see Subsubsection~3.13.6 for details. %%

\bye

% end of mnguide.tex

